Test Automation Maturity Improves Product Quality -- Quantitative Study of Open Source Projects Using Continuous Integration

The popularity of continuous integration (CI) is increasing as a result of market pressure to release product features or updates frequently. The ability of CI to deliver quality at speed depends on reliable test automation. In this paper, we present an empirical study to observe the effect of test automation maturity (assessed by standard best practices in the literature) on product quality, test automation effort, and release cycle in the CI context of open source projects. We run our test automation maturity survey and got responses from 37 open source java projects. We also mined software repositories of the same projects. The main results of regression analysis reveal that, higher levels of test automation maturity are positively associated with higher product quality (p-value=0.000624) and shorter release cycle (p-value=0.01891); There is no statistically significant evidence of increased test automation effort due to higher levels of test automation maturity and product quality. Thus, we conclude that, a potential benefit of improving test automation maturity (using standard best practices) is product quality improvement and release cycle acceleration in the CI context of open source projects. We encourage future research to extend our findings by adding more datasets with different programming languages and CI tools, closed source projects, and large-scale industrial projects. Our recommendation to practitioners (in the similar CI context) is to utilize standard best practices to improve test automation maturity.

==> sec/RTables.tex <==
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
fork & 37 & 5,212.838 & 15,225.550 & 10 & 159 & 709 & 86,000 \\ 
comment2021 & 27 & 59,807.780 & 102,196.000 & 765.000 & 9,067.000 & 53,058.000 & 505,912.000 \\ 
blank2021 & 27 & 44,112.180 & 77,853.560 & 703.000 & 9,795.000 & 49,111.500 & 385,483.000 \\ 
psize\_012020 & 37 & 199,094.300 & 327,200.300 & 3,113 & 27,093 & 210,661 & 1,421,621 \\ 
psize\_012021 & 37 & 229,234.200 & 398,647.300 & 3,479 & 36,987 & 221,079 & 1,868,078 \\ 
incr\_psize & 37 & 30,139.920 & 79,269.010 & 217 & 1,150 & 18,364 & 446,457 \\ 
ta\_size\_012020 & 37 & 28,471.700 & 55,846.830 & 836 & 5,311 & 29,866 & 324,003 \\ 
ta\_size\_012021 & 37 & 35,324.300 & 76,271.210 & 1,221 & 6,553 & 31,911 & 451,116 \\ 
incr\_ta\_size & 37 & 6,852.595 & 21,120.510 & 17 & 454 & 3,711 & 127,113 \\ 
project\_age & 37 & 3,765.378 & 1,051.079 & 578 & 3,271 & 4,024 & 6,782 \\ 
ctri\_ave\_m & 37 & 5.135 & 5.213 & 1 & 2 & 8 & 27 \\ 
ctri.m.peak & 28 & 12.786 & 19.758 & 1.000 & 3.750 & 16.250 & 107.000 \\ 
n\_testruns & 37 & 73,201,805.000 & 423,868,732.000 & 440 & 45,694 & 1,768,462 & 2,581,175,248 \\ 
t\_runs\_per\_m & 2 & 43,883.120 & 59,512.170 & 1,801.667 & 22,842.400 & 64,923.850 & 85,964.580 \\ 
exc\_times & 37 & 2,517,660.000 & 8,079,574.000 & 3,078 & 35,619 & 1,570,848 & 48,158,813 \\ 
n\_bugs & 37 & 121.324 & 364.112 & 2 & 9 & 84 & 2,181 \\ 
...21 & 32 & 38.750 & 77.525 & 0.000 & 2.750 & 33.000 & 381.000 \\ 
avgCCN & 37 & 1.997 & 0.639 & 1.200 & 1.600 & 2.300 & 4.600 \\ 
avg\_token & 37 & 60.257 & 14.674 & 32.100 & 47.800 & 68.800 & 104.700 \\ 
funCnt & 37 & 12,588.840 & 23,058.290 & 328 & 2,060 & 11,290 & 127,874 \\ 
code.duplicate.rate & 5 & 50.414 & 25.004 & 9.720 & 46.390 & 64.650 & 74.640 \\ 
code\_uniq\_rate & 37 & 86.809 & 9.527 & 53.870 & 84.460 & 92.210 & 96.380 \\ 
n\_release & 37 & 8.757 & 7.429 & 1 & 3 & 13 & 29 \\ 
bug\_precent & 37 & 2.730 & 1.575 & 1 & 1 & 4 & 5 \\ 
n\_bugs\_2 & 37 & 153.378 & 362.135 & 5 & 23 & 130 & 2,181 \\ 
TA\_maturity & 37 & 61.865 & 12.383 & 30 & 52 & 70 & 84 \\ 
TA\_maturity\_3 & 21 & 54.476 & 13.482 & 30.000 & 45.000 & 66.000 & 74.000 \\ 
defect\_density & 37 & 0.566 & 0.699 & 0.037 & 0.142 & 0.680 & 3.737 \\ 
incr\_ta\_size\_minmax & 37 & 6.325 & 16.452 & 1.000 & 1.340 & 3.877 & 100.000 \\ 
exc\_times\_minmax & 37 & 6.170 & 16.610 & 1.000 & 1.067 & 4.223 & 100.000 \\ 
cost & 37 & 12.494 & 32.433 & 2.029 & 2.603 & 10.222 & 200.000 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 

==> sec/background_v1.tex <==
\subsection{related work}

At the time of writing this paper, there do not exist empirical studies working on our research question. As noted by many sources, the need of evaluating the effect of achieving high level of test automation maturity as suggested by current test maturity models on product quality and trade-offs exist. Prior researchers indicated such a need, as they argued that, once the effect is validated, software organizations in the industry can get hints to improve the level of their test automation maturity.


Many studies has been performed to depict relationships among test automation maturity (the maturity of test automation practices), test automation effort, release cycle, and product quality. A summary of these relevant studies is in Table \ref{tab:related_work}. Column `Variables' shows which variables are observed in the study. Column 'Finding' presents the study finding(s) that pointed  the association relationship among observed variables.  

%However, the main obstacle prevent prior researchers is that, the widely used test maturity models focus on both manual testing and test automation and each model focuses on distinct key areas of test automation. Thus, before the evaluation, there is a need to collect  

%However, a lot of research has already been performed to investigate the effect of achieving high level of software process maturity as assessed by a popular maturity CMMi on product quality and trade-offs. As test automation is a software testing process that is a type of software process, we further studied such research on software process maturity  


%However, a lot of research has already been performed to investigate the effect of achieving high level of software process maturity as assessed by software process maturity models on higher product quality and trade-offs. A software process is a set of related activities to develop a software product.  Therefore, we studied prior research on software process maturity   


%As described in Table, the relevant studies can be divided into two set: (1) experience report based on direct experience of test automation projects by practitioners; (2) empirical studies based on direct observation by researchers. Only two empirical studies pointed out the association relationship among observed variables using the specific number.

\begin{table}[H]
\scriptsize
\centering
\caption{Control variables}\label{tab:related_work}
\begin{tabular}{|l | l |p{2.8cm} | p{2.8cm} |p{2.7cm}| p{4cm}| }
\hline
	Study & Year & Observation & Methodology & Variables  & Findings \\ \hline
	
	\cite{wang2020} & 2020 & %Test automation maturity improvement at a DevOps team from a Finnish software company 
	One DevOps team from F-secure (a Finnish software company) 
	& Experience report (based on meetings and a collection of experience notes, team reflection reports and telemetry result reports). & Test automaton maturity; release cycle; product quality  & Based on 10-year experience of test automation maturity improvement, this DevOps team  reported several observations: best practices in the literature were not suitable for their context, since adopting such best practices need the considerable effort;  Based on the team's experience, test automaton maturity improvement has the positive effect on accelerate release cycles and improving product quality.\\ \hline
	
	
	%concluded several critical success factors for its test automation maturity improvement, e.g., the whole team effort, expert team members, product testability. 
	
	\cite{hilton2017trade} & 2015 & 16 software developers from 14 different organizations & Interviews & Test automation maturity; product quality; test automation costs & This study observed that, in practical CI contexts, test automation maturity causes better product quality at the cost of increased efforts to design rigorous automated tests and execute them in frequent builds . \\ \hline
	
	\cite{khomh2012faster} & 2012 & 
	%Do faster releases improve software Quality when Mozilla and Firefox transitioned to a shorter release cycle during a period (2010-11) 
	The software development process of Mozilla Firefox during a period when it transitioned to a shorter release cycle 
	& Literature review; Case study (based on data mined from project wiki, project repository, crash repository, bug repository). 
	& Release cycle; Product quality 
	& This study found that, based on prior literature, short release cycles may negatively affect the product quality of software systems - since there is less time for both manual and automated testing. However, in the case of Mozilla Firefox, this study did not found significant association between release cycle and product quality.  \\\hline
	
	%& Literature review and case study & The conventional thought believe that short release cycles negatively affect the product quality of software systems - since there is less time for testing. However, in the case of Mozilla and Firefox, there is no significant association between release cycle and product quality.  \\\hline
	
    \cite{williams2009} & 2009 
    & One Microsoft team consisting of 32 developers & Case study based on software repository mining, survey, interview, and action research 
    & Product quality; Test automation costs
    & In the observed team, the software product quality improved at a cost of approximately 30\% more development time, when test automation is conducted incrementally with test-driven development. \\ \hline
    
    %\cite{ramler2006economic} & 2006 & The growing test automation efforts in iterative development to ensure product quality

    \cite{kasurinen2010software} & 2009  & 55 testing specialists from 31 organizations & Interviews &  Test automation maturity; test automation costs & Test automation practices requires the considerable efforts (in terms of planning efforts, design efforts, execution efforts, result analysis efforts) to be mature. \\ \hline
    
    \cite{berner2005} & 2005 & 5 practical test automation projects the authors have involved in & Experience report & Test automation maturity; release cycle; product quality & Test automation maturity achieved by several best practices (include defining a good test automation strategy, carefully designing and reusing automated tests, and building a testable SUT for testablity) can lead to shorter release cycles and better product quality. \\ \hline
%https://www.ics.uci.edu/~seal/publications/2020_ASE_Empirical.pdf
    \end{tabular}
\end{table}

%The study \cite{wang2020} presented the 10-year experience of test automation maturity improvement of one DevOps team at a Finnish software company F-secure. This DevOps team has successfully conducted test automation maturity improvement and gained the benefits (rapid release cycles, high product quality, and improved development productivity). It concluded several critical factors that determine the success of its test automation maturity improvement. These critical factors were grouped into four dimensions: Human, organizing, Technical, Process.  Each critical factor addressed by what practices in the observed team was described. 

%The study \cite{hilton2017trade} explored the state of CI practices by interviewing 16 developers from 14 different software organizations. As an important finding, the study reported that software organizations face the challenge ``to ensure that their code is correctly tested with manageable building times''. As reported by 86\% of software developers, in their organizations, the better product quality were achieved by test automation maturity improvement coming at the cost of increased efforts to develop rigours automated tests and execute them in frequent builds. 

%The study \cite{khomh2012faster} did an empirical case study on the software development process of Mozilla Firefox during the period when it transitioned to short release cycles in 2010 and 2011. This study observes does the length of the release cycle affect product quality, the duration of the bug fixing, and product updates. It collected metrics related data from the project wiki, project repository, crash repository, and bug repository of Mozilla Firefox. Descriptive statistics were used to analyze the collected metric data. One important study finding showed that, in the case of Mozilla Firefox, it did not find a significant association between the length of the release cycle and product quality.

%\paragraph{\textbf{Test automation maturity - Test automation effort}} Though 2 studies have found  that the higher level of test automation maturity was associated with increased test automation effort, their findings could not answer our research question \textit{``RQ1.Does achieve higher levels of test automation maturity (against standard best practices defined in current test maturity models) lead to the increased test automation effort in the CI context?''.} These 2 studies have observed that Test automation practices requires the  considerable efforts (in terms of planning efforts, design efforts, execution efforts, result analysis efforts) to be mature.

%5 studies have depicted the relationship between test automation maturity and test automation effort in a practical context.  The findings of these studies are contradicted, see Table. In an experience report, authors reported that, in the observed DevOps team, achieving higher levels of test automation maturity has lead to the increased test automation effort; The increased test automation effort was expended on adopting disciplined test automation practices against best practices suggested by test maturity models TPI, TMap. 

%Study \cite{wang2020} found that the higher level of test automation maturity was associated with increased test automation effort. In this study, authors observed that, adopting disciplined test automation practices (including define an explicit test automation strategy, measure test automation with right metrics, select right test tools to fit the current need, define clear guidelines to design and execute automated) to achieve high level of test automation maturity has lead to the increased test automation effort in the CI context. On the contrary, 



%adopting disciplined test automation practices (including define an explicit test automation strategy, measure test automation with right metrics, select right test tools, define a clear guidelines to design and execute automated) may lead to the increased test automation effort in the CI context. However, study presented different view. It observed that, even though the considerable early test automation effort is required to adopt standard disciplined practices in the CI context, but later achieved effort savings may offset the investment of early effort. Study also pointed that the same view as Study, but it focused on the general context instead of CI context of software development. The higher level of test automation maturity indicates more 
  

%\paragraph{\textbf{Test automation maturity - Release cycle}}

Under further investigation, we found that the above relevant studies are sufficient to answer our research question \textit{``Does test automation maturity (achieved by the adoption of disciplined best practices) lead to better product quality with a trade-off of increased test automation costs and longer under CI context?"} for many reasons.


First, our research question intends to explore the effect of mature test automation practices against standard best practices in test maturity models in the CI context in practice. This means we actually aims to explore the adoption of standard best practices defined in current test maturity models, and validate whether or not such standard best practices should be recommended for CI practitioners. However, among our identified studied, only study \cite{berner2005} has the similar aim.  In study \cite{berner2005}, authors reported that maturing test automation practices using several best practices (include defining a good test automation strategy, carefully designing and reusing automated tests, and building a testable SUT for testablity)  can lead to benefits - shorter release cycles and product quality. However, its finding was just based on authors' individual experience of 5 test automation projects and may not represent other sites. Besides, many best practices defined in existing test maturity models were not mentioned in their study, e.g., selecting right test tools, prioritizing important automated test for execution, providing enough resources. 

%our identified prior studies have the different understanding for the high maturity of test automation practices. Study and , considered the most mature test automation practices as the ones that can meet the current needs of the organization. 

%the observed team has its own understanding about mature test automation practices; This team considered the most mature test automation practices as the ones that can meet the current needs of the team. In study, high maturity of test automation practices 

Second, in all studies that have investigated how the maturity of test automation practices affect product quality, the findings verified the positive impact, see findings of study \cite{wang2020,berner2005,hilton2017trade} in Table \ref{tab:related_work}. However, all these studies concluded the findings based on qualitative evidence - the experience of individual practitioners. Study \cite{wang2020,berner2005} reported the experience of individual practitioners Study~\cite{hilton2017trade} interviewed individual practitioners. However, in SE research, qualitative evidence is valuable for exploring the reasons or details. To evaluate the fact and represent the overall picture of the software industry, cross-site quantitative evidence is needed. From this perspective, to confirm the positive effect of the maturity of test automation practices on product quality in practice, it is important to gather quantitative evidence from different sites.


Third, the findings of prior studies declared the conflict of viewpoints to answer our research question. The first conflict of viewpoint is about ``Does mature test automation practices lead do better product with a trade-off of increased test automation effort''. Study reported that maturing test automation practices expand more test automation effort. However, study presented different view. It observed that, even though the considerable test automation effort is required to achieve high level of test automation maturity, but the achieved effort savings may offset the investment of test automation effort. The second conflict of viewpoint is about ``Does mature test automation practices would lead do better product quality with a trade-off of release cycle time''. Study reported that maturing test automation practices lead to better product quality and shorter release cycles. Their findings indicate that maturing test automation practices would lead to better product quality but not trade-off the release cycle time. However, study observed that, achieving higher level of test automation maturity need more test automation effort and the increased test automation effort would cause the delay of product releases. In light of above conflict viewpoints,  to illustrate the consistent answer for our research question, the further evaluation study is needed. 


Moreover, 

%the trade-offs (in terms of testing efforts and release cycle time) of test automation maturity improvement to ensure high product quality were barely observed. One can see that, in all studies that have investigated how test automation maturity affect product quality, the findings noted the positive impact. The findings of these studies indicates that the high level of test automation maturity is associated with product quality in practice. However, only study \cite{williams2009} considered test automation costs as such a trade-off, however, its finding was just based on a team consisting of 32 developers at Microsoft and cannot represent other sites.





%In all studies that have investigated how test automation maturity affect product quality, the findings noted the positive impact. However, only study and study mentioned which disciplined best practices contribute to their test automation maturity improvement. These 2 studies are experience reports. They concluded best practices of test automation based on authors' experience in their working context. Their best practices may not fit the working contexts of other organizations. 


%\paragraph{\textbf{Lack of attention on trade-offs}} In all studies investigating test automation maturity (in form of practice maturity) and its impact on product quality, the findings pointed the positive relationship. However, the trade-offs (in forms of testing efforts and release cycle time) for maturing test automation practices were barely observed. Only study    \cite{williams2009} considered such trade-offs, however, its finding was just based on a team consisting of 32 developers at Microsoft and cannot represent other sites. 


The novelty of our study in this paper include: 
\begin{itemize}
    \item Our study has the direct objective to observe the effect of test automation maturity on product quality and its trade-offs in form of testing efforts and release cycle time. 
    
    \item Our study collected empirical evidence from open source projects by surveying their practitioners and mining their repositories. Software repository mining methodology was not used in prior studies. 

    
    \item Our study was recently finished and intended to present the current view for this research scope. Most of prior studies were published in several years ago. Only \cite{wang2020} is a recent study, and that is an experience report.
    
    \item Findings: 
\end{itemize}

==> sec/relatedwork.tex <==
\noindent To study related work, a systematic literature review was conducted  following "Guidelines for performing SLRs in SE" from \cite{keele2007guidelines}. 
